Towards a new paradigm for assistive technology at home: research challenges, design issues and performance assessment

Providing elderly and people with special needs, including those suffering from physical disabilities and chronic diseases, with the possibility of retaining their independence at best is one of the most important challenges our society is expected to face. Assistance models based on the home care paradigm are being adopted rapidly in almost all industrialized and emerging countries. Such paradigms hypothesize that it is necessary to ensure that the so-called Activities of Daily Living are correctly and regularly performed by the assisted person to increase the perception of an improved quality of life. This chapter describes the computational inference engine at the core of Arianna, a system able to understand whether an assisted person performs a given set of ADL and to motivate him/her in performing them through a speech-mediated motivational dialogue, using a set of nearables to be installed in an apartment, plus a wearable to be worn or fit in garments.

==> resourceImg.tex <==
\begin{figure*}[!b]
	\centering
	\begin{minipage}{0.80\linewidth}
		\centering
		\includegraphics[width=1\linewidth]{./images/jconsole.pdf} % .eps
	\end{minipage}
	\hfill
	\begin{minipage}{0.17\linewidth}
		\centering
		\begin{small}
			\begin{tabular}{r|cc}
				\textit{test}				& \textit{memory}	& \textit{$\eta$}	\\ \hline
				\coloredBox{Res1}		& 2 GB 				& 1 					\\
				\coloredBox{Res2} 	& 4 GB 				& 1 					\\
				\coloredBox{Res3} 	& 1 GB 			 	& 1.3 				\\
				\coloredBox{Res4}		& 2 GB 				& 2					
			\end{tabular}
		\end{small}
		\captionof{figure}{\small The resources required by the system during four experiments performed on the same dataset, with the above configurations.}
		\label{fig:jConsole}
	\end{minipage}
\end{figure*}


